BEND 2.0: Benchmarking the Capabilities Needed to Design DNA

Genomic foundation models are increasingly used to propose DNA sequences and edits. But successful design requires capabilities that current benchmarks do not measure. Here we introduce BEND 2.0 (BENchmark for DNA language models), which tests how well models predict the effects of DNA changes and whether these predictions can guide sequence design. Across eight tasks built on five experimental datasets, we find that model choice and how representations are accessed both affect performance. Linear readouts fitted to frozen representations can match or exceed models' native outputs, and functional post-training substantially improves the models' capabilities. Linear readouts transfer well across experimental assays and genes, suggesting that models capture functional patterns beyond the data used to fit individual predictors. At the same time, strong prediction of average effects can conceal weaker prediction of context-specific effects, and accurate prediction of combined mutation effects does not imply accurate prediction of their interactions. In design tasks, model predictions can reduce the number of candidates needed to find a desired response, but still leave substantial room for better design choices, particularly for context-specific and multi-cell objectives. Our benchmark reveals that genomic models now display signs of general utility but have yet to saturate on performance in even simple tasks.

==> author-affiliations.tex <==
\RequirePackage{pdfrender}
\pdfgentounicode=1
\pdfglyphtounicode{tfm:psyr/heart}{2661}
\pdfglyphtounicode{tfm:psyr/club}{2667}
\pdfglyphtounicode{tfm:psyr/spade}{2664}
\pdfglyphtounicode{tfm:fa5free1regular/envelope}{2709}
\font\affcopyfont=psyr at 6.25pt
\newcommand{\affsuit}[2]{%
  \smash{\rlap{\textpdfrender{TextRenderingMode=Invisible}{%
    \affcopyfont\char#2\relax}}}%
  \includegraphics[height=6.25pt]{author-suits/#1-outline.pdf}}
\newcommand{\affmark}[1]{\rlap{\textsuperscript{\kern.12em#1}}}
\newcommand{\KU}{\affsuit{heart}{169}}
\newcommand{\DTU}{\affsuit{club}{167}}
\newcommand{\NOVO}{\affsuit{spade}{170}}
\newcommand{\corrEnvelope}{\raisebox{.2pt}{\fontsize{6.2}{6.2}\selectfont\faEnvelope[regular]}}
\newcommand{\CORR}{\kern.35em\corrEnvelope}
\newcommand{\authorEmail}[2][]{%
  \makebox[0pt][c]{\normalfont\fontsize{9}{11}\selectfont\textcolor{black}{#2\rlap{#1}}}}
\newcommand{\paperAuthorBlock}{%
  \begin{minipage}[t]{\dimexpr\textwidth-2\tabcolsep\relax}
    \centering
    \fontsize{10.5}{14}\selectfont\bfseries
    \makebox[\linewidth][c]{%
    \hspace*{16.2pt}%
    \begin{tabular}{@{}*{3}{>{\centering\arraybackslash}p{140pt}@{}}}
      Andreas Bjerregaard\affmark{\KU} & Rachael DeVries\affmark{\KU\kern.16em\NOVO} & Dionysia Danai Brilli\affmark{\KU} \\[-3pt]
      \authorEmail[\CORR]{anje@di.ku.dk} & \authorEmail{rachael.devries@bio.ku.dk} & \authorEmail{danai.brilli@bio.ku.dk} \\[4pt]
      Panagiotis Antoniadis\affmark{\KU} & Yan Li\affmark{\KU} & Anders Krogh\affmark{\KU} \\[-3pt]
      \authorEmail{panagiotis.antoniadis@bio.ku.dk} & \authorEmail{yanli@di.ku.dk} & \authorEmail{akrogh@di.ku.dk} \\[4pt]
      Wouter Boomsma\affmark{\KU} & Ole Winther\affmark{\KU\kern.16em\DTU} & Frederikke Isa Marin\affmark{\KU} \\[-3pt]
      \authorEmail[\CORR]{wb@di.ku.dk} & \authorEmail[\CORR]{ole.winther@bio.ku.dk} & \authorEmail[\CORR]{frma@di.ku.dk}
    \end{tabular}}\par
    \vspace{7pt}
    {\normalfont\fontsize{9}{11}\selectfont
      \KU\hspace{.3em}University of Copenhagen\hspace{1.0em}%
      \DTU\hspace{.3em}Technical University of Denmark\hspace{1.0em}%
      \NOVO\hspace{.3em}Novo Nordisk A/S\par
      \vspace{3pt}
      \corrEnvelope\hspace{.4em}Corresponding authors\par}
  \end{minipage}%
}
\author{\paperAuthorBlock}


==> preprint-style.tex <==
\RequirePackage{etoolbox}
\makeatletter
\newcommand{\bend@headerfont}{\normalfont\normalsize\color{black}}
\newcommand{\iclrpreprintcopy}{%
  \iclrfinalcopy
  \fancypagestyle{bendfirst}{%
    \fancyhead{}%
    \fancyhead[L]{\bend@headerfont BEND 2.0}%
    \fancyhead[R]{\bend@headerfont Preprint}%
  }%
  \patchcmd{\@maketitle}%
    {\lhead{Published as a conference paper at ICLR 2027}}%
    {\lhead{\bend@headerfont\ifodd\value{page}%
         BEND 2.0%
       \else Benchmarking the Capabilities Needed to Design DNA\fi}%
     \rhead{\bend@headerfont Preprint}%
     \thispagestyle{bendfirst}}%
    {}%
    {\PackageError{preprint-style}{Could not set the preprint header}%
      {Check the title definition in the bundled ICLR style.}}%
  \renewcommand{\headrulewidth}{0.35pt}%
  \let\bend@headrule\headrule
  \renewcommand{\headrule}{{\color{black!75}\bend@headrule}}%
  \patchcmd{\@maketitle}%
    {\hsize\textwidth}%
    {\hsize\textwidth\vskip-18pt\relax}%
    {}%
    {\PackageError{preprint-style}{Could not adjust the title position}%
      {Check the title definition in the bundled ICLR style.}}%
  \patchcmd{\@maketitle}%
    {\@title\par}%
    {\@title\par\vskip3pt}%
    {}%
    {\PackageError{preprint-style}{Could not adjust the title-to-author gap}%
      {Check the title definition in the bundled ICLR style.}}%
  \patchcmd{\@maketitle}%
    {\vskip 0.3in minus 0.1in}%
    {\vskip\dimexpr0.3in-6pt\relax minus 0.1in}%
    {}%
    {\PackageError{preprint-style}{Could not adjust the space before Abstract}%
      {Check the title definition in the bundled ICLR style.}}%
}
\makeatother

